Sublinear-Time Computation in the Presence of Online Erasures

We initiate the study of sublinear-time algorithms that access their input via an online adversarial erasure oracle. After answering each input query, such an oracle can erase $t$ input values. Our goal is to understand the complexity of basic computational tasks in extremely adversarial situations, where the algorithm's access to data is blocked during the execution of the algorithm in response to its actions. Specifically, we focus on property testing in the model with online erasures. We show that two fundamental properties of functions, linearity and quadraticity, can be tested for constant $t$ with asymptotically the same complexity as in the standard property testing model. For linearity testing, we prove tight bounds in terms of $t$, showing that the query complexity is $\Theta(\log t).$ In contrast to linearity and quadraticity, some other properties, including sortedness and the Lipschitz property of sequences, cannot be tested at all, even for $t=1$. Our investigation leads to a deeper understanding of the structure of violations of linearity and other widely studied properties. We also consider implications of our results for algorithms that are resilient to online adversarial corruptions instead of erasures.

==> tocspecial.tex <==
%% tocspecial.tex 2020-09-01  Version 0.22  ToC style file
%------------------------------------------------------------------
% Filename: tocspecial.cls
% 
% This documentclass is intended for typesetting articles for the
% 
% Theory of Computing.
% 
% See http://theoryofcomputing.org for further details.
%
% Version 0.1 Initial combination of banners from previous style files.
% Version 0.2 Addition of CCC banners. Clean up.
% Version 0.21 Addition of more CCC banners, up to 2023
% Version 0.22 Rename \boolean --> \aboolean to avoid clash with ifthen.
% ------------------------------------------------------------------
%
%% Special issue banners:

%% explanation: BC = 2012 BD = 2013 ... CA = 2020 CB = 2021 ...

\newcommand{\motwani}{Special issue in honor of Rajeev Motwani}
\newcommand{\aboolean}{Special issue: Analysis of Boolean Functions}
\newcommand{\approxrandomBC}{Special issue: APPROX-RANDOM 2012}
\newcommand{\approxrandomBD}{Special issue: APPROX-RANDOM 2013}
\newcommand{\approxrandomBE}{Special issue: APPROX-RANDOM 2014}
\newcommand{\approxrandomBF}{Special issue: APPROX-RANDOM 2015}
\newcommand{\approxrandomBG}{Special issue: APPROX-RANDOM 2016}
\newcommand{\randomBI}{Special issue: RANDOM 2018}
\newcommand{\approxrandomBJ}{Special issue: APPROX-RANDOM 2019}
\newcommand{\cccBF}{Special issue: CCC 2015}
\newcommand{\cccBG}{Special issue: CCC 2016}
\newcommand{\cccBH}{Special issue: CCC 2017}
\newcommand{\cccBI}{Special issue: CCC 2018}
\newcommand{\cccBJ}{Special issue: CCC 2019}
\newcommand{\cccCA}{Special issue: CCC 2020}
\newcommand{\cccCB}{Special issue: CCC 2021}
\newcommand{\cccCC}{Special issue: CCC 2022}
\newcommand{\cccCD}{Special issue: CCC 2023}

